SVRecon: Sparse Voxel Rasterization for Surface Reconstruction

We extend the recently proposed sparse voxel rasterization paradigm to the task of high-fidelity surface reconstruction by integrating Signed Distance Function (SDF), named SVRecon. Unlike 3D Gaussians, sparse voxels are spatially disentangled from their neighbors and have sharp boundaries, which makes them prone to local minima during optimization. Although SDF values provide a naturally smooth and continuous geometric field, preserving this smoothness across independently parameterized sparse voxels is nontrivial. To address this challenge, we promote coherent and smooth voxel-wise structure through (1) robust geometric initialization using a visual geometry model and (2) a spatial smoothness loss that enforces coherent relationships across parent-child and sibling voxel groups. Extensive experiments across various benchmarks show that our method achieves strong reconstruction accuracy while having consistently speedy convergence. The code will be made public.

==> figs/3_sdf_sign_assignment/3_sdf_sign_assignment.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.95\linewidth]{figs/3_sdf_sign_assignment/figure2.pdf}
    \caption{sign assignment based visibility}
    \label{fig:sign_assignment}
\end{figure}

==> figs/4_voxel_association/4_voxel_association.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.95\linewidth]{figs/4_voxel_association/Figure3.pdf}
    \caption{voxel association using fine cell unit}
    \label{fig:placeholder}
\end{figure}

==> sec/4_4_progressive_voxel_allocation.tex <==
%

==> sec/legacy/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

Please follow the steps outlined below when submitting your manuscript to the IEEE Computer Society Press.
This style guide now has several important modifications (for example, you are no longer warned against the use of sticky tape to attach your artwork to the paper), so all authors should read this new version.

%-------------------------------------------------------------------------
\subsection{Language}

All manuscripts must be in English.

\subsection{Dual submission}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a
discussion of the policy on dual submissions.

\subsection{Paper length}
Papers, excluding the references section, must be no longer than eight pages in length.
The references section will not be included in the page count, and there is no limit on the length of the references section.
For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
{\bf There will be no extra page charges for \confName\ \confYear.}

Overlength papers will simply not be reviewed.
This includes papers where margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
Note that this \LaTeX\ guide already sets the figure captions and references in a smaller font.
The reason why such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
The review process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in 11 pages.

%-------------------------------------------------------------------------
\subsection{The ruler}
The \LaTeX\ style defines a printed ruler that should be present in the version submitted for review.
The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
If you are preparing a document using a non-\LaTeX\ document preparation system, arrange for an equivalent ruler to appear on the final output pages.
The presence or absence of the ruler should not change the appearance of any other content on the page.
The camera-ready copy should not contain a ruler.
(\LaTeX\ users may use the options of \texttt{cvpr.sty} to switch between different versions.)

Reviewers:
note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
Use fractional references (\eg, this line is $087.5$), although in most cases the approximate location would be adequate.


\subsection{Paper ID}
Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


\subsection{Mathematics}

Please, number all of your sections and displayed equations as in these examples:
\begin{equation}
  E = m\cdot c^2
  \label{eq:important}
\end{equation}
and
\begin{equation}
  v = a\cdot t.
  \label{eq:also-important}
\end{equation}
It is important for the reader to be able to refer to any particular equation.
Just because you did not refer to it in the text does not mean that some future reader might not need to refer to it.
It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
(Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
All authors will benefit from reading Mermin's description of how to write mathematics:
\url{http://www.pamitc.org/documents/mermin.pdf}.

\subsection{Blind review}

Many authors misunderstand the concept of anonymizing for blind review.
Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
That is all.
(But see below for tech reports.)

Saying ``this builds on the work of Lucy Smith [1]'' does not mean that you are Lucy Smith;
it says that you are building on her work.
If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

An example of a bad paper just asking to be rejected:
\begin{quote}
\begin{center}
    An analysis of the frobnicatable foo filter.
\end{center}

   In this paper, we present a performance analysis of our previous paper [1], and show that it is inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}


An example of an acceptable paper:
\begin{quote}
\begin{center}
     An analysis of the frobnicatable foo filter.
\end{center}

   In this paper, we present a performance analysis of the paper of Smith \etal [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time that covers similar or overlapping material, you may need to refer to that submission to explain the differences, just as you would if you had previously published related work.
In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
\begin{quote}
[1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be found elsewhere and refer them to a technical report.
For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
Then submit the tech report as supplemental material.
Again, do not assume that the reviewers will read this material.

Sometimes your paper is about a problem that you tested using a tool that is widely known to be restricted to a single institution.
For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the 1970 audience would like to hear about your
solution.
The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.
Do not write ``We show how to improve our previous work [Anonymous, 1968].
This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors.
Instead write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.
   This system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
   Ours handles it by including a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
   It displayed the following behaviours, which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
A reviewer might think that it is likely that the new article was written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been contracted to solve problem B.
\medskip

\noindent
FAQ\medskip\\
{\bf Q:} Are acknowledgements OK?\\
{\bf A:} No.  Leave them for the final copy.\medskip\\
{\bf Q:} How do I cite my results reported in open challenges?
{\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
However, for your results, you should not identify yourself and should not mention your participation in the challenge.
Instead, present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison with other results.\medskip\\

\begin{figure}[t]
  \centering
  \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}

   \caption{Example of caption.
   It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
   \label{fig:onecol}
\end{figure}

\subsection{Miscellaneous}

\noindent
Compare the following:\\
\begin{tabular}{ll}
 \verb'$conf_a$' &  $conf_a$ \\
 \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
\end{tabular}\\
See The \TeX book, p165.

The space after \eg, meaning ``for example'', should not be a sentence-ending space.
So \eg is correct, {\em e.g.} is not.
The provided \verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
However, use it only when there are three or more authors.
Thus, the following is correct:
   ``Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has only two authors.

\begin{figure*}
  \centering
  \begin{subfigure}{0.68\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{An example of a subfigure.}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.28\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Another example of a subfigure.}
    \label{fig:short-b}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}


==> sec/legacy/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
The columns should be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered, and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

The captions of the figures and tables should be in 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centered.  Table captions should be above tables, while figure captions should be below figures.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period, and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use the footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example, at the beginning of the sentence, you can use
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, include the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When citing multiple papers at once, make sure that you cite them in numerical order such as this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \caption{Results.   Ours is better.}
  \label{tab:example}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead, use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise and, therefore, must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it is almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence, avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/legacy/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> sec/legacy/Method.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% SH
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \subsection{Voxel initialization using pointmap}
% \label{subsec:voxel_initialization_using_pointmap}

% A robust initialization of the Signed Distance Function (SDF) grid is crucial for efficiently optimizing a sparse voxel-based surface representation from scratch. 
% Existing initialization strategies, however, are ill-suited for this task. 
% Simple heuristics like sphere initialization fail to capture complex object topology. 
% View-dependent methods like TSDF fusion, which were designed for dense data, produce a discontinuous SDF field when applied to sparse points, as the sign can flip abruptly between adjacent voxels. This violates the continuity essential for gradient-based optimization.
% Conversely, recent learning-based approaches are computationally expensive, and their high precision is superfluous for an initial estimate. 
% Therefore, we require an initialization strategy that is fast, view-independent, and generates a globally continuous SDF field sufficient to guide the optimization.

% To meet these requirements, we propose an initialization strategy based on the geometric density of the SfM point cloud. 
% Our approach is guided by the principle that the initial SDF need not be perfectly accurate, but must robustly localize the zero-level-set. 
% This is achieved by assigning values based on local point density in two steps:
% \begin{enumerate}
%     \item \textbf{Point Cloud Denoising:} Raw SfM point clouds often contain significant noise and sparse outliers. We first apply the DBSCAN algorithm to filter the point cloud, retaining only the largest and most coherent cluster of points $\mathcal{P}$. This step ensures that our initialization is not corrupted by erroneous points.
    
%     \item \textbf{Density-based SDF Assignment:} We structure the denoised points $\mathcal{P}$ into a K-D Tree for efficient spatial queries. For each voxel center $\mathbf{p}$ in our grid, we count the number of SfM points, $N_{\text{neighbors}}$, within a query radius $r$ (e.g., twice the voxel size). The SDF value at $\mathbf{p}$ is then assigned based on this local density:
%     \begin{equation}
%         \text{SDF}(\mathbf{p}) = 
%         \begin{cases} 
%             \text{dist}(\mathbf{p}, \mathcal{P}) - r & \text{if } N_{\text{neighbors}} \geq N_{\text{min}} \\
%             \text{dist}(\mathbf{p}, \mathcal{P}) & \text{if } N_{\text{neighbors}} < N_{\text{min}}
%         \end{cases}
%         \label{eq:sdf_init_revised}
%     \end{equation}
%     where $N_{\text{min}}$ is a minimum density threshold (e.g., $N_{\text{min}}=3$), and $\text{dist}(\mathbf{p}, \mathcal{P})$ is the Euclidean distance from $\mathbf{p}$ to its nearest point in the SfM cloud $\mathcal{P}$. This assigns a negative value inside dense regions by subtracting the larger search radius from the smaller nearest-neighbor distance.
% \end{enumerate}
% This two-step process proves to be both fast, initializing a typical scene in approximately 5 seconds, and view-independent.
% The resulting initialization provides a stable yet minimal geometric guide by seeding a thin surface shell exclusively in the densest regions of the SfM point cloud. 
% This coarse anchor is crucial as it allows the network to autonomously learn and converge to a high-fidelity surface, rather than being constrained by an inaccurate, fully-formed initial shape.



% \subsection{SDF Learning in Sparse Voxels}
% \label{sec:sdf_learning}

% In our explicit voxel-based SDF representation, the value at any point within a voxel is derived from the trilinear interpolation of the SDF values stored at its eight vertices.
% A naive rendering approach might sample the SDF only at the ray's entry and exit points for each traversed voxel. 
% However, this is problematic. Since both sample points are interpolated from the \textit{same eight vertices}, the optimization becomes a severely under-constrained problem for each voxel. 
% While gradients flow to all eight vertices, the sparse information from only two internal samples is insufficient to resolve their values unambiguously, leading to noisy, rough surfaces that cling to voxel boundaries.

% To address this, we introduce a midpoint-based rendering strategy that enforces inter-voxel consistency, acting as a powerful regularizer. 
% Instead of sampling within a single voxel, we compute opacity based on the SDF values at the midpoints of two \textit{consecutive} voxels along a ray. 
% This couples adjacent voxels within the rendering process. The opacity $\alpha_i$ for the interval between the current midpoint $t_i$ and the next $t_{i+1}$ is computed using a formulation adapted from NeuS~\cite{neus_paper_citation}:
% \begin{equation}
%     \alpha_i = \max\!\left(
%       \frac{\phi(f(t_i)) - \phi(f(t_{i+1}))}{\phi(f(t_i))},\, 0
%     \right),
%     \label{eq:opacity}
% \end{equation}
% where $f(t)$ is the interpolated SDF value at position $t$, and $\phi$ is the logistic density function. This design ensures that the gradient from a single opacity calculation propagates to the vertices of two neighboring voxels (up to 16 vertices in total), forcing the learned SDF field to be smooth and continuous across voxel boundaries.

% A challenge of this inter-voxel approach is color determination, as the rendered color now depends on two voxels, $\mathbf{v}_i$ and $\mathbf{v}_{i+1}$, which store colors $\mathbf{c}_i$ and $\mathbf{c}_{i+1}$. 
% We solve this by blending their colors based on the precise surface location. 
% If a sign change is detected between $t_i$ and $t_{i+1}$, we find the exact zero-crossing point $t_{surf}$ via linear interpolation. The final surface color $\mathbf{c}_{surf}$ is then a weighted average of the two voxels' colors:
% \begin{equation}
%     \mathbf{c}_{surf} = (1 - w) \cdot \mathbf{c}_i + w \cdot \mathbf{c}_{i+1},
%     \quad \text{where} \quad
%     w = \frac{t_{surf} - t_i}{t_{i+1} - t_i}.
%     \label{eq:color_blending}
% \end{equation}
% This blending strategy ensures smooth color transitions, preventing blocky artifacts at voxel boundaries.

% In summary, our midpoint-based rendering, combined with the color blending scheme, provides dense gradient propagation across voxel neighborhoods. This acts as a strong implicit regularization, leading to more stable training and the reconstruction of sharp, well-regularized surfaces.


% \subsection{Voxel Refinement with SDF Criteria}

% In the SDF mode, refinement alternates between two operations:
% \emph{pruning} empty voxels and \emph{subdividing} surface voxels. Both are
% scheduled periodically during training, combining the coarse-to-fine idea
% with the original SVRaster refinement strategy.

% \paragraph{Pruning.}
% We prune voxels every 1000 iterations to discard regions that are unlikely to
% contain a surface. A voxel is removed if all eight corner SDF values share the
% same sign (no surface crossing), or if all absolute SDF magnitudes exceed a
% threshold. The threshold depends on the scale parameter $\log s$, which in NeuS
% controls the sharpness of the logistic function $\Phi_s$. A larger $\log s$
% shrinks the ``learning thickness'' band around the zero level set, so that
% only voxels contributing above a small fraction (e.g., $>1\%$ of rendering
% weights) are retained.

% \paragraph{Subdivision.}
% Every 1000 iterations, we also subdivide voxels that are likely to contain
% surfaces. In the SDF mode, a voxel is subdivided if its corner values show a
% sign change, ensuring that only surface-relevant voxels are refined.
% Additionally, every 3000 iterations we increase the maximum octree depth,
% implementing a coarse-to-fine schedule: the voxel grid starts coarse and is
% progressively refined as training proceeds, so that the representation
% follows surface adjustments while controlling memory usage.

% Overall, pruning aggressively eliminates empty voxels, while subdivision
% gradually increases resolution only around surfaces. This hybrid scheme
% combines SVRaster’s efficient pruning/subdivision pipeline with an SDF-aware
% coarse-to-fine schedule, yielding compact yet geometrically accurate voxel
% structures that track surfaces throughout training.

% \subsection{Grid--Voxel Mapping and Neighbor Search}
% To enable continuous propagation of regularization losses (e.g., Eikonal, smoothness, Laplacian) across space, we introduce a three-part data structure that explicitly links grid cells (fine resolution sampling points) with voxels (coarse sparse blocks). This mapping allows the system to efficiently query spatial neighbors and enforce differential constraints.

% \paragraph{Data Structures}
% \begin{enumerate}
%     \item \textbf{Dense Bitmask (A)}:  
%     A boolean array of size $G^3$ ($G=2^n$, where $n$ is the maximum subdivision level) marking whether each grid coordinate is covered by any voxel.
%     Acts as a global occupancy mask for the grid, enabling $O(1)$ checks of whether a location is valid.

%     \item \textbf{Compact Index Table (B)}:  
%     A linear array storing only valid grid indices in ascending order.
%     Built from (A) using prefix-sum compaction, ensuring memory efficiency while retaining ordering.
%     Querying the position of a grid index within this table requires binary search, yielding $O(\log M)$ time (where $M$ is the number of valid grid cells).

%     \item \textbf{Voxel Index Mapping (C)}:  
%     For each valid grid index in (B), we store the voxel index that owns this grid point.
%     Each grid cell belongs to exactly one voxel, guaranteeing uniqueness and avoiding conflicts.
%     Retrieval from this mapping is $O(1)$ once the compacted index is known.
% \end{enumerate}

% \paragraph{Neighbor Query}
% Given a grid coordinate:
% \begin{enumerate}
%     \item Validity Check: Query (A) $\rightarrow O(1)$.
%     \item Index Localization: If valid, binary search (B) to find the compacted position $\rightarrow O(\log M)$.
%     \item Voxel Retrieval: Use (C) to obtain the corresponding voxel index $\rightarrow O(1)$.
% \end{enumerate}

% Therefore, fetching the 6 neighbors of a grid coordinate costs $O(6 \log M) \approx O(\log M)$.  
% On the GPU, these queries are executed in parallel across thousands of threads, so in practice the effective cost approaches constant time.

% \paragraph{Advantages}
% \begin{itemize}
%     \item \textbf{Loss Propagation Continuity}: Ensures that regularization terms applied at the grid level naturally propagate across voxel boundaries.
%     \item \textbf{GPU Efficiency}: Combination of dense mask and compacted table balances memory usage (sparse storage) with parallel-friendly random access.
%     \item \textbf{Scalability}: While voxels are stored adaptively and sparsely, the dense grid is always defined at the finest subdivision level. This independence allows fine-grained regularization to be applied consistently, even in regions represented by large voxels.
% \end{itemize}




% \subsection{Regularization Losses}

% \subsubsection{Eikonal Loss (numerical gradient)}
% We enforce the gradient norm of the SDF to be close to 1.  
% For each grid coordinate $x_i$, the gradient is approximated by central differences:

% \begin{align}
% \partial_x f(x_i) &= 
% \frac{f(x_i+\epsilon_x) - f(x_i-\epsilon_x)}{2\epsilon}, \\
% \partial_y f(x_i) &\;\text{and}\; 
% \partial_z f(x_i)\;\;\text{similarly.} \nonumber
% \end{align}


% The loss is then
% \begin{equation}
% L_{\text{eik}} = \frac{1}{N}\sum_{i=1}^N \Bigl|\,\|\nabla f(x_i)\|_2 - 1\,\Bigr|.
% \end{equation}

% \subsubsection{Smoothness Loss (second-order Laplacian)}
% We regularize the second derivatives so that curvature vanishes, similar to Neuralangelo.  
% At each grid coordinate $x_i$, the Laplacian is estimated with second-order finite differences:

% \begin{align}
% \nabla^{2} f(x_i) \;\approx\;
% &\;\frac{f(x_i+\epsilon_x) - 2f(x_i) + f(x_i-\epsilon_x)}{\epsilon^2} \nonumber \\
% &+ \frac{f(x_i+\epsilon_y) - 2f(x_i) + f(x_i-\epsilon_y)}{\epsilon^2} \nonumber \\
% &+ \frac{f(x_i+\epsilon_z) - 2f(x_i) + f(x_i-\epsilon_z)}{\epsilon^2}.
% \end{align}


% The smoothness loss is then
% \begin{equation}
% L_{\text{smooth}} = \frac{1}{N}\sum_{i=1}^N \bigl|\,\nabla^{2} f(x_i)\,\bigr|.
% \end{equation}

% \subsubsection{Random Sampling within Grid Cells}
% Both eikonal and smoothness losses are also evaluated at random positions inside each grid cell:

% \begin{equation}
% x' = x + \delta, \qquad \delta \sim \mathcal{U}(0.0, 1.0)\cdot h,
% \end{equation}

% where $h$ is the grid spacing.  
% This stochastic sampling improved stability and resulted in sharper and less noisy geometry in our experiments.

